Point Separation and Obstacle Removal by Finding and Hitting Odd Cycles

Suppose we are given a pair of points $s, t$ and a set $S$ of $n$ geometric objects in the plane, called obstacles. We show that in polynomial time one can construct an auxiliary (multi-)graph $G$ with vertex set $S$ and every edge labeled from $\{0, 1\}$, such that a set $S_d \subseteq S$ of obstacles separates $s$ from $t$ if and only if $G[S_d]$ contains a cycle whose sum of labels is odd. Using this structural characterization of separating sets of obstacles we obtain the following algorithmic results. In the Obstacle-Removal problem the task is to find a curve in the plane connecting s to t intersecting at most q obstacles. We give a $2.3146^qn^{O(1)}$ algorithm for Obstacle-Removal, significantly improving upon the previously best known $q^{O(q^3)} n^{O(1)}$ algorithm of Eiben and Lokshtanov (SoCG'20). We also obtain an alternative proof of a constant factor approximation algorithm for Obstacle-Removal, substantially simplifying the arguments of Kumar et al. (SODA'21). In the Generalized Points-Separation problem, the input consists of the set S of obstacles, a point set A of k points and p pairs $(s_1, t_1),... (s_p, t_p)$ of points from A. The task is to find a minimum subset $S_r \subseteq S$ such that for every $i$, every curve from $s_i$ to $t_i$ intersects at least one obstacle in $S_r$. We obtain $2^{O(p)} n^{O(k)}$-time algorithm for Generalized Points-Separation problem. This resolves an open problem of Cabello and Giannopoulos (SoCG'13), who asked about the existence of such an algorithm for the special case where $(s_1, t_1), ... (s_p, t_p)$ contains all the pairs of points in A. Finally, we improve the running time of our algorithm to $f(p,k) n^{O(\sqrt{k})}$ when the obstacles are unit disks, where $f(p,k) = 2^O(p) k^{O(k)}$, and show that, assuming the Exponential Time Hypothesis (ETH), the running time dependence on $k$ of our algorithms is essentially optimal.

==> Makefile <==
TEXSRC := document.tex
AUX := $(TEXSRC:.tex=.aux)
PDF := $(TEXSRC:.tex=.pdf)

all:
	pdflatex $(TEXSRC)
	-bibtex $(AUX)
	-pdflatex $(TEXSRC)
	-pdflatex $(TEXSRC)
	\rm -f *.aux *.log *.bbl *.blg *.out *.vtc 

clean:
	\rm -f *.aux *.log *.bbl *.blg *.pdf *.vtc *.out 




==> socg-22-overleaf/introduction.tex <==
Suppose we are given a set $\cs$ of geometric objects in the plane, and we want to modify $\cs$ in order to achieve certain guarantees on coverage of paths between a fixed set $A$ of points.
Such problems have received  significant interest in both sensor networks~\cite{balister2009trap, KumarLA05, BeregK09, ChanK12}, robotics~\cite{lavalle, eiben2018improved} and 
computational geometry~\cite{Eiben2017, mcp-fpt, bksvCGTA}. There have been two closely related lines of work on this topic:
\textbf{(i)} \emph{remove} a \textit{smallest} number of obstacles from $\cs$ so that the points $A$
are no longer pairwise separated, and \textbf{(ii)} \emph{retain} a \textit{smallest} number of obstacles so that the points $A$ still remain pairwise separated. 
The former is called the \obstacleremoval{} problem whereas the latter is called \pointsep{}.


\subsection*{Our Results}

\begin{itemize}
    \item An alternative algorithm for 2-\pointsep{}.

    \item Improved FPT algorithm for \obstacleremoval{} parameterized by the number of intersected obstacles. That is, we give an algorithm that
    finds an $s$--$t$ path intersecting at most $q$ obstacles in $2.3416^q n^{O(1)}$ time.

    \item Simplify the constant factor approximation for \obstacleremoval{} by Kumar et al.~\cite{mcp2021}.

    \item A $2^{O(p)} n^{O(k)}$-time algorithm for \gptsep{} and improve it to $f(p,k) \cdot n^{O(\sqrt{k})}$ when the obstacles
    are unit disks, where $f(p,k) = 2^{O(p)} k^{O(k)}$. We also show that these algorithms are near optimal assuming the Exponential Time Hypothesis (ETH).
\end{itemize}

\textbf{TODO: Coherent story linking all our rseults}


==> socg-22-overleaf/labeled-graphs.tex <==

We begin my describing the construction of the labeled intersection graph $G_\cs=(\cs, X)$ of the
obstacles $\cs$. For the ease of exposition, we will use $S$ to refer to the obstacle $S \in \cs$ 
as well as the vertex for $S$ in $G_\cs$ interchangeably. 


\subparagraph*{Constructing the graph $G_\cs$} For every obstacle $S \in \cs$ we first select an arbitrary point $\refp(S) \in S$
and designate it to be the \emph{reference point} of the obstacle. 
Next, we select the \emph{reference curve} $\pi$ to be an arbitrary curve in the plane connecting $s$ and $t$. 
For every pair of obstacles $S, S' \in \cs$ that intersect, we add edges to $G$ as follows.
\begin{itemize}
    \item Add an edge $e_0 = (S, S')$ with $\lab(e_0) = 0$ if there exists a path between $\refp(S)$ and $\refp(S')$ contained
        in the region $S \cup S'$ that crosses $\pi$ an \emph{even} number of times.
    \item Add an edge $e_1 = (S, S')$ with $\lab(e_1) = 1$ if there exists a path between $\refp(S)$ and $\refp(S')$ contained
        in the region $S \cup S'$ that crosses $\pi$ an \emph{odd} number of times.
\end{itemize}

Checking whether there exists a path between $\refp(S)$ and $\refp(S')$ that crosses $\pi$ and odd (resp. even)
number of times can be done in time linear in the size of arrangement $\Arr(S \cup S' \cup \pi)$. Assuming that
$|\Arr(\cs)| = n^{O(1)}$, the graph $G_\cs$ can be constructed in $n^{O(1)}$ time.

Next we prove the following structural property of the graph $G_\cs$.

\begin{lemma}
    \label{lem:odd-cycle}
    A set of obstacles $\cs' \subseteq S$ in the graph $G_\cs$ separates the points $s$ and $t$ if and only if 
    the induced graph $H = G_\cs[\cs']$ contains an odd labeled cycle.
\end{lemma}

\begin{proof}
    $(\Rightarrow)$ For the forward direction, suppose we are given a set of obstacles $\cs'$ that separate $s$ from $t$.
    Let $\cr_\cs' = \bigcup_{S \in \cs'} S$ be the region bounded by all obstacles.
    Since $s, t$ lie in the exterior of all obstacles, they also lie outside the region $\cr_\cs'$.
    Clearly $s, t$ must lie in different connected regions $R_s, R_t$ of $\mathbb{R}^2 - \cr(\cs')$ or else 
    the set $\cs'$ would not separate them.
    At least one of $R_s$ or $R_t$ must be bounded, wlog assume it is $R_s$. Let $\gamma'$ be the closed 
    curve that is the common boundary of $\cr(\cs')$ and $R_s$. Clearly, $\gamma'$ encloses $s$ but not $t$
    and therefore separates $s$ from $t$. Using Fact~\ref{fact-separate}, we obtain that $\gamma'$ intersects
    the reference curve $\pi$ an odd number of times. Observe that the curve $\gamma' = \alpha_1, \alpha_2, \dots, \alpha_r$
    consists of multiple \emph{sections} where each section $\alpha_i$ is part of the boundary of some obstacle $S_i$. 
    For each of these sections $\alpha_i$, we add a \emph{detour} $\delta_i = q_i \rightarrow \refp(S_i) \rightarrow q_i$ 
    where $q_i$ is an arbitrary point on $\alpha_i$. We ensure that the curve $\delta_i$ stays within the obstacle $S_i$.
    Let $\gamma$ be the path obtained by adding these detours to $\gamma'$.
    Since every detour crosses the reference curve $\pi$ zero or two (an even number) of times, the modified curve $\gamma$
    also crosses $\pi$ an odd number of times. We will now translate the curve $\gamma$ to a \emph{walk} in the labeled
    intersection graph $G_\cs$. Specifically, consider the section of curve $\gamma_{i,i+1} = \refp(S_i) \rightarrow q_i \rightarrow q_{i+1} \rightarrow \refp(S_{i+1})$
    between two consecutive detours. Therefore the obstacles $S_i, S_{i+1}$ must intersect and there exists a path $\gamma_{i,i+1}$
    connecting their reference points contained in $S_i \cup S_{i+1}$ that intersects the reference curve $\pi$ and odd (resp. even) number of times. By construction,
    $G\cs$ must contain an edge $e_{i, i+1}$ with label $1$ (resp. 0).  By replacing all these sections of $\gamma$ with the corresponding edges
    of $G_\cs$ we obtain an odd-labeled closed walk $W$ in $G_\cs$. Note that this is a walk because an obstacle can occur on the curve $\gamma'$ multiple times.
    Of all the odd-labeled closed sub-walks of $W$, we select one that is inclusion minimal. This gives a simple odd-labeled cycle in $G_\cs$.

    $(\Leftarrow)$ For the reverse direction, we can translate the odd-labeled cycle to a closed curve in the plane by replacing every edge
    $e_i = (S, S')$ by the path in the plane $\gamma_i$ connecting the reference points $\refp(S)$ and $\refp(S')$ with that crosses the reference curve 
    $\pi$ consistent with $\lab(e_i)$.
    This gives us a closed curve $\gamma$ in the plane that crosses $\pi$ an odd number of times but this curve may be self intersecting. Let $X$ be the
    set of all the reference points and all the intersection points on $\gamma$. Consider the \emph{plane graph} $G_\gamma$ whose vertices are points in $X$
    and edges are simple subpaths $\gamma(x_i, x_{i+1})$ of $\gamma$ connecting consecutive points $x_i, x_{i+1}$ on $\gamma$. 
    We label each edge as $0$ or $1$ depending upon the number of times the curve $\gamma(x_i, x_{i+1})$ crosses $\pi$. The curve $\gamma$
    translates to an odd-labeled closed walk $W$ in $G_\gamma$. Same as before, chosing an inclusion minimal odd-labeled closed sub-walk
    gives us a simple odd labeled cycle which in turn gives us a simple closed curve in the plane that crosses $\pi$ an odd number of times.
    From Fact~\ref{fact-separate}, it follows that $\cs'$ separates $s$ and $t$.
\end{proof}

\subparagraph{\boldmath 2-\pointsep{} as Shortest Odd Cycle in $G_\cs$} From Lemma~\ref{lem:odd-cycle}, it follows that a minimum set of obstacles that separates $s$ from $t$
corresponds to an odd-labeled cycle in $G_\cs$ with fewest vertices. This readily gives a polytime lagorithm for 2-\pointsep{}. Specifically, 
for a fixed starting vertex, we can compute the shortest odd cycle in $G_\cs$ in $O(|\cs|^2)$ time by performing BFS on an unlabeled 
auxiliary graph $G'$ with vertex set is $\cs \times \{0, 1\}$. For every edge $e = (S, S')$ of $G_\cs$,
we add edges $\{(S, 0), (S', 0)\}$ and $\{(S, 1), (S',1)\}$ if $\lab(e) = 0$. Otherwise, we add the edges $\{(S, 0), (S', 1)\}$ and $\{(S, 1), (S',0)\}$.
Repeating over all starting vertices gives the shortest odd cycle in $G_\cs$.

\subsection{Application to \obstacleremoval{}}
We will show how to cast \obstacleremoval{} as a Labeled Odd Cycle Transversal problem on the graph $G_\cs$.
Recall that in \obstacleremoval{} problem, we want to remove a set $\cs_d \subseteq \cs$
of obstacles from the input so that $s$ and $t$ are connected. Equivalently, we want to select a subset $\cs_d$ of obstacles such that the complement set $\cs - \cs_d$ \emph{does not
separate} $s$ and $t$. From Lemma~\ref{lem:odd-cycle}, it follows that the obstacles $\cs - \cs_d$ do not separate $s$ and $t$ if and only if $G_\cs[\cs - \cs_d]$ does not contain
an odd labeled cycle. 
This gives us the following important lemma.
\begin{lemma}
    \label{lemma:obstacle-removal}
    A set of obstacles $\cs_d$ is an optimal solution to \obstacleremoval{} if and only if the set of vertices $\cs_d$ is the smallest odd cycle transversal of $G_\cs$. 
\end{lemma}
This allows us to apply the vast set of existing results for odd cycle transversal to obstacle removal problems.
In particular, this readily gives an improved algorithm for \obstacleremoval when parameterized by the solution size (number of removed obstacles).
Let $G_\cs^+$ denote the graph $G_\cs$ where every edge $e$ with $\lab(e) = 0$ is subdivided. Clearly an odd-labeled cycle in $G_\cs$ has
odd length in $G_\cs^+$ and vice versa.
Applying the FPT algorithm for odd cycle transversal from~\cite{oct-fpt} on the graph $G_\cs^+$ gives us the following result.
\begin{theorem}
    There exists a $2.3146^k n^{O(1)}$ algorithm for \obstacleremoval{} parameterized by $k$, the number of removed obstacles.
\end{theorem}

This also gives us an $O(\log n)$ approximation for \obstacleremoval{} by using the $O(\log n)$-approximation for odd cycle transversal on graph $G_\cs^+$.
Observe that instances of obstacle removal are special cases of odd cycle transversal, specifically where the graph $G_\cs$ is an intersection graph of obstacles.
By applying known results on decomposition of \emph{region intersection graphs}, we can obtain a constant approximation for such instances. The following algorithm
significantly simplifies the constant approximation algorithm for \obstacleremoval{} from~\cite{mcp2021}.

\subsubsection*{Constant Approximation for \obstacleremoval{}}
At a high level, our algorithm is based on formulating an LP for labeled odd cycle transversal and then applying known rounding techniques. 
Let $x_i \in \{0, 1\}$ be a binary variable that denotes whether obstacle $S_i$ is included to the solution or not.



==> socg-22-overleaf/prelims.tex <==

The previous work have defined the \pointsep{} and \obstacleremoval{} in terms of graph problems on a i\emph{color-connected planar
graph}. Specifically, given an arrangement $\Arr(\cs)$ of obstacles $\cs$, we consider the dual graph $G_\Arr = (V, E)$ of the 
arrangement whose vertices are faces of $\Arr(\cs)$ and edges connect neighboring faces. Next we define a coloring function 
$\textsf{col} : V \rightarrow  2^{\cs}$ which assigns every vertex to the set of obstacles containing it. That is, each obstacle corresponds to a unique color in this graph and therefore 
we can use them interchangeably. Since obstacles are connected regions, the set of vertices containing any given color is also connected.
We can also safely assume that $s$ and $t$ lie in the exterior of all obstacles because if not, an obstacle containing $s$ (or $t$) trivially
seperates them, and every $s$--$t$ path must intersect all such obstacles.

It is easy to see that an $s$--$t$ path in the plane that intersects fewest obstacles corresponds to a path in the graph that uses a minimum number of colors
in the colored graph $(G_\Arr, \col)$ and vice versa. 
The set of colors used by a path $\pi_{st}$ is defined as $\col(\pi_{st}) = \bigcup_{v \in \pi_{st}} \col(v)$.

We can also define 2-\pointsep as the problem of computing a \emph{min-color separator} of the graph $(G_\Arr, \col)$.
Let $V(S') \subseteq V$ be the set of vertices of $G_\Arr$ that contain at least one color from $S'$.
A set of colors $S_r \subseteq S$ is a \emph{color separator} if $s$ and $t$ are disconnected in $G_\Arr - V(S_r)$. 
Observe that every $s$--$t$ path must intersect at least one color in $S_r$. Therefore, a color separator of
minimum cardinality is a solution of 2-\pointsep, that is the minimum set of obstacles separating
$s$ from $t$.

The previous work~\cite{mcp2021} used structural properties of the colored graph $(G_\Arr, \col)$ to obtain a polytime algorithm
for \obstacleremoval{} and a constant approximation for \pointsep{}.
One key difference in our approach is that instead of working on the colored graph $(G_\Arr, \col)$, we found it
more convenient to work with a so-called \emph{labeled intersection graph} $(G_\cs, \lab)$ of obstacles which we will define later.
Roughly speaking, given a set of obstacles $\cs$ and a \emph{reference curve} $\pi$ in the plane connecting $s$ and $t$, 
we build a multi-graph where vertices are obstacles in $\cs$ and edges connect a pair of intersecting obstacles. 
Every edge $e \in E$ is assigned a \emph{parity} label $\mathsf{lab}(e) \in \{0, 1\}$  based on the reference curve $\pi$. 
We say that a path is labeled \emph{odd} (or \emph{even}) if the sum of labels of its edges is odd (or even) respectively.

Once this graph is constructed, we can forget about obstacles and formulate our problems using just the parity labels $\lab(e)$ on the
edges of $G_\cs$. Since the parity function is much simpler to work with compared to the color function, this allows us to
significantly simplify the results from~\cite{mcp2021} and obtain new results.
In the next section, we describe the construction of graph $G_\cs$ and prove some structural results that allow us to 
cast 2-\pointsep{} as finding shortest odd labeled cycle in $G_\cs$ and \obstacleremoval{} as the smallest odd cycle
transversal of $G_\cs$. We will need the following important property of plane curves.

\subparagraph{Plane curves} A \textit{plane curve} (or simply \textit{curve}) is specified by a continuous function $\pi:[0,1] \rightarrow \mathbb{R}^2$, 
where the points $\pi(0)$ and $\pi(1)$ are called the \textit{endpoints} (for convenience, we also use the notation $\pi$ to denote the image of the path function $\pi$).
A curve is \textit{simple} if it is injective, and is \textit{closed} if its two endpoints are the same.
We say a curve $\pi$ \textit{separates} a pair $(a,b)$ of two points in $\mathbb{R}^2$ if $a$ and $b$ belong to different connected components of $\mathbb{R}^2 \backslash \pi$.
\begin{fact} \label{fact-separate}
Let $\pi$ be a curve with endpoints $a,b \in \mathbb{R}^2$.
A simple closed curve $\gamma$ separates $(a,b)$ iff $\pi$ crosses $\gamma$ an odd number of times.
A closed curve $\gamma$ separates $(a,b)$ if $\pi$ crosses $\gamma$ an odd number of times.
\end{fact}


